Resource-Efficient Invariant Networks: Exponential Gains by Unrolled Optimization

Achieving invariance to nuisance transformations is a fundamental challenge in the construction of robust and reliable vision systems. Existing approaches to invariance scale exponentially with the dimension of the family of transformations, making them unable to cope with natural variabilities in visual data such as changes in pose and perspective. We identify a common limitation of these approaches--they rely on sampling to traverse the high-dimensional space of transformations--and propose a new computational primitive for building invariant networks based instead on optimization, which in many scenarios provides a provably more efficient method for high-dimensional exploration than sampling. We provide empirical and theoretical corroboration of the efficiency gains and soundness of our proposed method, and demonstrate its utility in constructing an efficient invariant network for a simple hierarchical object detection task when combined with unrolled optimization. Code for our networks and experiments is available at https://github.com/sdbuch/refine.

==> tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_OUTPUT_MODE	u-ctags	/u-ctags or e-ctags/
!_TAG_PROGRAM_AUTHOR	Universal Ctags Team	//
!_TAG_PROGRAM_NAME	Universal Ctags	/Derived from Exuberant Ctags/
!_TAG_PROGRAM_URL	https://ctags.io/	/official site/
!_TAG_PROGRAM_VERSION	0.0.0	/2614dbe/
10.1093/mnras/stv632	refs.bib	/^@article{10.1093\/mnras\/stv632,$/;"	e
10.5555/2969442.2969465	refs.bib	/^@inproceedings{10.5555\/2969442.2969465,$/;"	e
10.5555/3327546.3327581	refs.bib	/^@inproceedings{10.5555\/3327546.3327581,$/;"	e
8667888	refs.bib	/^@ARTICLE{8667888,$/;"	e
8747339	refs.bib	/^@INPROCEEDINGS{8747339,$/;"	e
9420272	refs.bib	/^@ARTICLE{9420272,$/;"	e
A. L. Samuel	example/example_paper.bib	/^  author = 	 "A. L. Samuel",$/;"	a
A. Newell and P. S. Rosenbloom	example/example_paper.bib	/^  author =       "A. Newell and P. S. Rosenbloom",$/;"	a
Aharon Azulay and Yair Weiss	refs.bib	/^  author  = {Aharon Azulay and Yair Weiss},$/;"	a
Alaifari, Rima and Alberti, Giovanni S and Gauksson, Tandri	refs.bib	/^  author    = "Alaifari, Rima and Alberti, Giovanni S and Gauksson, Tandri",$/;"	a
Alaifari2018-ef	refs.bib	/^@INPROCEEDINGS{Alaifari2018-ef,$/;"	e
Alcorn2018-qg	refs.bib	/^@INPROCEEDINGS{Alcorn2018-qg,$/;"	e
Alpher02	example/egbib.bib	/^@article{Alpher02,$/;"	e
Alpher03	example/egbib.bib	/^@article{Alpher03,$/;"	e
Alpher04	example/egbib.bib	/^@article{Alpher04,$/;"	e
Alpher05	example/egbib.bib	/^@inproceedings{Alpher05,$/;"	e
Anandan, P	refs.bib	/^  author  = "Anandan, P",$/;"	a
Anandan1989-su	refs.bib	/^@ARTICLE{Anandan1989-su,$/;"	e
Andrew Brock and Jeff Donahue and Karen Simonyan	refs.bib	/^author={Andrew Brock and Jeff Donahue and Karen Simonyan},$/;"	a
Aric A. Hagberg and Daniel A. Schult and Pieter J. Swart	refs.bib	/^  author =       {Aric A. Hagberg and Daniel A. Schult and Pieter J. Swart},$/;"	a
Author, N. N.	example/example_paper.bib	/^  author= {Author, N. N.},$/;"	a
Authors14	example/egbib.bib	/^@misc{Authors14,$/;"	e
Authors14b	example/egbib.bib	/^@misc{Authors14b,$/;"	e
Azulay2018-nm	refs.bib	/^@article{Azulay2018-nm,$/;"	e
Baker, Simon and Matthews, Iain	refs.bib	/^  author  = "Baker, Simon and Matthews, Iain",$/;"	a
Baker2004-fh	refs.bib	/^@ARTICLE{Baker2004-fh,$/;"	e
Bar, Leah and Sapiro, Guillermo	refs.bib	/^  author    = "Bar, Leah and Sapiro, Guillermo",$/;"	a
Bar2010-iq	refs.bib	/^@INPROCEEDINGS{Bar2010-iq,$/;"	e
Basri, Ronen and Jacobs, David W	refs.bib	/^  author    = "Basri, Ronen and Jacobs, David W",$/;"	a
Basri2017-vn	refs.bib	/^@INPROCEEDINGS{Basri2017-vn,$/;"	e
Belhumeur, P N and Kriegman, D J	refs.bib	/^  author    = "Belhumeur, P N and Kriegman, D J",$/;"	a
Belhumeur1996-ae	refs.bib	/^@INPROCEEDINGS{Belhumeur1996-ae,$/;"	e
Bronstein2021-un	refs.bib	/^@ARTICLE{Bronstein2021-un,$/;"	e
Brown, Lisa Gottesfeld	refs.bib	/^  author    = "Brown, Lisa Gottesfeld",$/;"	a
Brown1992-vz	refs.bib	/^@ARTICLE{Brown1992-vz,$/;"	e
Bruna, Joan and Mallat, St{\\'e}phane	refs.bib	/^  author   = "Bruna, Joan and Mallat, St{\\'e}phane",$/;"	a
Bruna2013-on	refs.bib	/^@ARTICLE{Bruna2013-on,$/;"	e
Buchanan, S and Haque, T and Kinget, P and Wright, J	refs.bib	/^  author    = "Buchanan, S and Haque, T and Kinget, P and Wright, J",$/;"	a
Buchanan2018-ip	refs.bib	/^@INPROCEEDINGS{Buchanan2018-ip,$/;"	e
Carmon2021-rl	refs.bib	/^@ARTICLE{Carmon2021-rl,$/;"	e
Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey	refs.bib	/^  author =       {Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey},$/;"	a
Chen, Xiaohan and Liu, Jialin and Wang, Zhangyang and Yin, Wotao	refs.bib	/^author = {Chen, Xiaohan and Liu, Jialin and Wang, Zhangyang and Yin, Wotao},$/;"	a
Chen2019-eq	refs.bib	/^@ARTICLE{Chen2019-eq,$/;"	e
Chen2020-bl	refs.bib	/^@InProceedings{Chen2020-bl,$/;"	e
Chen2021-un	refs.bib	/^@ARTICLE{Chen2021-un,$/;"	e
Cire{\\c s}an, Dan and Meier, Ueli and Schmidhuber, Juergen	refs.bib	/^author = "Cire{\\c s}an, Dan and Meier, Ueli and Schmidhuber, Juergen",$/;"	a
Cloninger2020-ov	refs.bib	/^@article{Cloninger2020-ov,$/;"	e
Cohen, Taco and Welling, Max	refs.bib	/^  author    = "Cohen, Taco and Welling, Max",$/;"	a
Cohen2016-vq	refs.bib	/^@INPROCEEDINGS{Cohen2016-vq,$/;"	e
Cohen2018-aj	refs.bib	/^@INPROCEEDINGS{Cohen2018-aj,$/;"	e
Cootes, T F and Edwards, G J and Taylor, C J	refs.bib	/^  author    = "Cootes, T F and Edwards, G J and Taylor, C J",$/;"	a
Cootes1998-sk	refs.bib	/^@INPROCEEDINGS{Cootes1998-sk,$/;"	e
Cubuk, Ekin D. and Zoph, Barret and Mane, Dandelion and Vasudevan, Vijay and Le, Quoc V.	refs.bib	/^author = {Cubuk, Ekin D. and Zoph, Barret and Mane, Dandelion and Vasudevan, Vijay and Le, Quoc /;"	a
Cubuk2018-yu	refs.bib	/^@InProceedings{Cubuk2018-yu,$/;"	e
DBLP:journals/corr/abs-2106-06418	refs.bib	/^@article{DBLP:journals\/corr\/abs-2106-06418,$/;"	e
Dai2017-lj	refs.bib	/^@INPROCEEDINGS{Dai2017-lj,$/;"	e
Dai2021-rg	refs.bib	/^@ARTICLE{Dai2021-rg,$/;"	e
Dieleman, Sander and Willett, Kyle W. and Dambre, Joni	refs.bib	/^    author = {Dieleman, Sander and Willett, Kyle W. and Dambre, Joni},$/;"	a
DudaHart2nd	example/example_paper.bib	/^@Book{DudaHart2nd,$/;"	e
Engstrom, Logan and Tran, Brandon and Tsipras, Dimitris and Schmidt, Ludwig and Madry, Aleksander	refs.bib	/^  author={Engstrom, Logan and Tran, Brandon and Tsipras, Dimitris and Schmidt, Ludwig and Madry,/;"	a
Engstrom2017-ps	refs.bib	/^@inproceedings{Engstrom2017-ps,$/;"	e
Fawzi, Alhussein and Frossard, Pascal	refs.bib	/^  author        = "Fawzi, Alhussein and Frossard, Pascal",$/;"	a
Fawzi, Alhussein and Frossard, Pascal	refs.bib	/^  author = {Fawzi, Alhussein and Frossard, Pascal},$/;"	a
Fawzi2015-ul	refs.bib	/^@ARTICLE{Fawzi2015-ul,$/;"	e
Fawzi:210209	refs.bib	/^@inproceedings{Fawzi:210209,$/;"	e
Felzenszwalb, Pedro and McAllester, David and Ramanan, Deva	refs.bib	/^  author    = "Felzenszwalb, Pedro and McAllester, David and Ramanan, Deva",$/;"	a
Felzenszwalb2008-ui	refs.bib	/^@INPROCEEDINGS{Felzenszwalb2008-ui,$/;"	e
Felzenszwalb2010-gv	refs.bib	/^@ARTICLE{Felzenszwalb2010-gv,$/;"	e
FirstName Alpher	example/egbib.bib	/^author = {FirstName Alpher},$/;"	a
FirstName Alpher and  FirstName Fotheringham-Smythe	example/egbib.bib	/^author = {FirstName Alpher and  FirstName Fotheringham-Smythe},$/;"	a
FirstName Alpher and FirstName Fotheringham-Smythe and FirstName Gamow	example/egbib.bib	/^author = {FirstName Alpher and FirstName Fotheringham-Smythe and FirstName Gamow},$/;"	a
FirstName Alpher and FirstName Gamow	example/egbib.bib	/^author = {FirstName Alpher and FirstName Gamow},$/;"	a
FirstName LastName	example/egbib.bib	/^ author = {FirstName LastName},$/;"	a
Geoffrey E Hinton and Sara Sabour and Nicholas Frosst	refs.bib	/^author={Geoffrey E Hinton and Sara Sabour and Nicholas Frosst},$/;"	a
Gilboa, Dar and Buchanan, Sam and Wright, John	refs.bib	/^  author    = "Gilboa, Dar and Buchanan, Sam and Wright, John",$/;"	a
Gilboa2019-px	refs.bib	/^@INPROCEEDINGS{Gilboa2019-px,$/;"	e
Girshick2015-qw	refs.bib	/^@INPROCEEDINGS{Girshick2015-qw,$/;"	e
Gregor, Karol and LeCun, Yann	refs.bib	/^  author    = "Gregor, Karol and LeCun, Yann",$/;"	a
Gregor2010-nh	refs.bib	/^@INPROCEEDINGS{Gregor2010-nh,$/;"	e
Hendrycks2019-ae	refs.bib	/^@INPROCEEDINGS{Hendrycks2019-ae,$/;"	e
Hinton, Geoffrey	refs.bib	/^  author        = "Hinton, Geoffrey",$/;"	a
Hinton, Geoffrey E and Krizhevsky, Alex and Wang, Sida D	refs.bib	/^  author    = "Hinton, Geoffrey E and Krizhevsky, Alex and Wang, Sida D",$/;"	a
Hinton2011-yb	refs.bib	/^@INPROCEEDINGS{Hinton2011-yb,$/;"	e
Hinton2021-fm	refs.bib	/^@ARTICLE{Hinton2021-fm,$/;"	e
Horn, Berthold K P and Schunck, Brian G	refs.bib	/^  author  = "Horn, Berthold K P and Schunck, Brian G",$/;"	a
Horn1981-by	refs.bib	/^@ARTICLE{Horn1981-by,$/;"	e
Jaderberg, Max and Simonyan, Karen and Zisserman, Andrew and Kavukcuoglu, Koray	refs.bib	/^author = {Jaderberg, Max and Simonyan, Karen and Zisserman, Andrew and Kavukcuoglu, Koray},$/;"	a
Jenatton2010-oj	refs.bib	/^@INPROCEEDINGS{Jenatton2010-oj,$/;"	e
Jialin Liu and Xiaohan Chen and Zhangyang Wang and Wotao Yin	refs.bib	/^author={Jialin Liu and Xiaohan Chen and Zhangyang Wang and Wotao Yin},$/;"	a
John Zarka and Louis Thiry and Tomas Angles and Stephane Mallat	refs.bib	/^author={John Zarka and Louis Thiry and Tomas Angles and Stephane Mallat},$/;"	a
KARYGIANNI2014232	refs.bib	/^@article{KARYGIANNI2014232,$/;"	e
Kanazawa, Angjoo and Sharma, Abhishek and Jacobs, David	refs.bib	/^  author        = "Kanazawa, Angjoo and Sharma, Abhishek and Jacobs, David",$/;"	a
Kanazawa, Angjoo and Zhang, Jason Y. and Felsen, Panna and Malik, Jitendra	refs.bib	/^  author = {Kanazawa, Angjoo and Zhang, Jason Y. and Felsen, Panna and Malik, Jitendra},$/;"	a
Kanazawa2014-zf	refs.bib	/^@ARTICLE{Kanazawa2014-zf,$/;"	e
Kanazawa_2019_CVPR	refs.bib	/^@INPROCEEDINGS{Kanazawa_2019_CVPR,$/;"	e
Kanbak, C and Moosavi-Dezfooli, S and Frossard, P	refs.bib	/^  author    = "Kanbak, C and Moosavi-Dezfooli, S and Frossard, P",$/;"	a
Kanbak2018-lw	refs.bib	/^@INPROCEEDINGS{Kanbak2018-lw,$/;"	e
Kellman, Michael R. and Bostan, Emrah and Repina, Nicole A. and Waller, Laura	refs.bib	/^  author={Kellman, Michael R. and Bostan, Emrah and Repina, Nicole A. and Waller, Laura},$/;"	a
Kellman, Michael and Bostan, Emrah and Chen, Michael and Waller, Laura	refs.bib	/^  author={Kellman, Michael and Bostan, Emrah and Chen, Michael and Waller, Laura},$/;"	a
Keys, R	refs.bib	/^  author   = "Keys, R",$/;"	a
Keys1981-jx	refs.bib	/^@ARTICLE{Keys1981-jx,$/;"	e
Kobler2017-wr	refs.bib	/^@INPROCEEDINGS{Kobler2017-wr,$/;"	e
Kondor, Risi and Trivedi, Shubhendu	refs.bib	/^  author =       {Kondor, Risi and Trivedi, Shubhendu},$/;"	a
Kosiorek, A R and Sabour, S and Teh, Y W and Hinton, G E	refs.bib	/^  author    = "Kosiorek, A R and Sabour, S and Teh, Y W and Hinton, G E",$/;"	a
Kosiorek2019-ow	refs.bib	/^@ARTICLE{Kosiorek2019-ow,$/;"	e
Kuo, Han-Wen and Zhang, Yuqian and Lau, Yenson and Wright, John	refs.bib	/^  author    = "Kuo, Han-Wen and Zhang, Yuqian and Lau, Yenson and Wright, John",$/;"	a
Kuo2019-as	refs.bib	/^@ARTICLE{Kuo2019-as,$/;"	e
Laptev, Dmitry and Savinov, Nikolay and Buhmann, Joachim M. and Pollefeys, Marc	refs.bib	/^  author = {Laptev, Dmitry and Savinov, Nikolay and Buhmann, Joachim M. and Pollefeys, Marc},$/;"	a
Laptev_2016_CVPR	refs.bib	/^@INPROCEEDINGS{Laptev_2016_CVPR,$/;"	e
Lefebure2001-uz	refs.bib	/^@ARTICLE{Lefebure2001-uz,$/;"	e
Lef{\\'e}bure, Martin and Cohen, Laurent D	refs.bib	/^  author  = "Lef{\\'e}bure, Martin and Cohen, Laurent D",$/;"	a
Lucas, Bruce D and Kanade, Takeo	refs.bib	/^  author    = "Lucas, Bruce D and Kanade, Takeo",$/;"	a
Lucas1981-ef	refs.bib	/^@INPROCEEDINGS{Lucas1981-ef,$/;"	e
M. J. Kearns	example/example_paper.bib	/^  author = {M. J. Kearns},$/;"	a
MachineLearningI	example/example_paper.bib	/^@Book{MachineLearningI,$/;"	e
Maintz, J B Antoine and Viergever, Max A	refs.bib	/^  author   = "Maintz, J B Antoine and Viergever, Max A",$/;"	a
Maintz1998-vz	refs.bib	/^@ARTICLE{Maintz1998-vz,$/;"	e
Mallat, St{\\'e}phane	refs.bib	/^  author    = "Mallat, St{\\'e}phane",$/;"	a
Mallat2012-sl	refs.bib	/^@ARTICLE{Mallat2012-sl,$/;"	e
Mobahi, Hossein and Zitnick, C Lawrence and Ma, Yi	refs.bib	/^  author    = "Mobahi, Hossein and Zitnick, C Lawrence and Ma, Yi",$/;"	a
Mobahi2012-to	refs.bib	/^@INPROCEEDINGS{Mobahi2012-to,$/;"	e
Muckley, Matthew J. and Riemenschneider, Bruno and Radmanesh, Alireza and Kim, Sunwoo and Jeong, Geunu and Ko, Jingyu and Jun, Yohan and Shin, Hyungseob and Hwang, Dosik and Mostapha, Mahmoud and Arberet, Simon and Nickel, Dominik and Ramzi, Zaccharie and Ciuciu, Philippe and Starck, Jean-Luc and Teuwen, Jonas and Karkalousos, Dimitrios and Zhang, Chaoping and Sriram, Anuroop and Huang, Zhengnan and Yakubova, Nafissa and Lui, Yvonne W. and Knoll, Florian	refs.bib	/^  author={Muckley, Matthew J. and Riemenschneider, Bruno and Radmanesh, Alireza and Kim, Sunwoo /;"	a
NEURIPS2019_9015	refs.bib	/^@incollection{NEURIPS2019_9015,$/;"	e
Nakada, Ryumei and Imaizumi, Masaaki	refs.bib	/^  author   = "Nakada, Ryumei and Imaizumi, Masaaki",$/;"	a
Nakada2019-jr	refs.bib	/^@ARTICLE{Nakada2019-jr,$/;"	e
Newell81	example/example_paper.bib	/^@InCollection{Newell81,$/;"	e
Ongie2020-pu	refs.bib	/^@ARTICLE{Ongie2020-pu,$/;"	e
Oyallon, Edouard and Belilovsky, Eugene and Zagoruyko, Sergey	refs.bib	/^author = {Oyallon, Edouard and Belilovsky, Eugene and Zagoruyko, Sergey},$/;"	a
Oyallon_2017_ICCV	refs.bib	/^@InProceedings{Oyallon_2017_ICCV,$/;"	e
P. Langley	example/example_paper.bib	/^ author    = {P. Langley},$/;"	a
Parikh, Neal and Boyd, Stephen	refs.bib	/^  author    = "Parikh, Neal and Boyd, Stephen",$/;"	a
Parikh2014-om	refs.bib	/^@ARTICLE{Parikh2014-om,$/;"	e
Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and Desmaison, Alban and Kopf, Andreas and Yang, Edward and DeVito, Zachary and Raison, Martin and Tejani, Alykhan and Chilamkurthy, Sasank and Steiner, Benoit and Fang, Lu and Bai, Junjie and Chintala, Soumith	refs.bib	/^author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James a/;"	a
Pedersoli2015-wx	refs.bib	/^@ARTICLE{Pedersoli2015-wx,$/;"	e
Qu, Qing and Li, Xiao and Zhu, Zhihui	refs.bib	/^  author    = "Qu, Qing and Li, Xiao and Zhu, Zhihui",$/;"	a
Qu2019-jf	refs.bib	/^@INPROCEEDINGS{Qu2019-jf,$/;"	e
R. O. Duda and P. E. Hart and D. G. Stork	example/example_paper.bib	/^  author =       "R. O. Duda and P. E. Hart and D. G. Stork",$/;"	a
Sabour2021-wt	refs.bib	/^@INPROCEEDINGS{Sabour2021-wt,$/;"	e
SabourFH17	refs.bib	/^@inproceedings{SabourFH17,$/;"	e
Samuel59	example/example_paper.bib	/^@Article{Samuel59,$/;"	e
Sara Sabour and Nicholas Frosst and Geoffrey E. Hinton	refs.bib	/^  author={Sara Sabour and Nicholas Frosst and Geoffrey E. Hinton},$/;"	a
Schmidt-Hieber, Johannes	refs.bib	/^  author        = "Schmidt-Hieber, Johannes",$/;"	a
Schmidt-Hieber2019-jt	refs.bib	/^@ARTICLE{Schmidt-Hieber2019-jt,$/;"	e
SciPyProceedings_11	refs.bib	/^@InProceedings{SciPyProceedings_11,$/;"	e
Simchowitz, Max and El Alaoui, Ahmed and Recht, Benjamin	refs.bib	/^  author        = "Simchowitz, Max and El Alaoui, Ahmed and Recht, Benjamin",$/;"	a
Simchowitz2017-pe	refs.bib	/^@ARTICLE{Simchowitz2017-pe,$/;"	e
Sofia Karygianni and Pascal Frossard	refs.bib	/^author = {Sofia Karygianni and Pascal Frossard},$/;"	a
Sohn, Kihyuk and Lee, Honglak	refs.bib	/^  author    = "Sohn, Kihyuk and Lee, Honglak",$/;"	a
Sohn2012-ml	refs.bib	/^@INPROCEEDINGS{Sohn2012-ml,$/;"	e
Song2021-gj	refs.bib	/^@INPROCEEDINGS{Song2021-gj,$/;"	e
Stein, Elias M and Weiss, Guido	refs.bib	/^  author    = "Stein, Elias M and Weiss, Guido",$/;"	a
Stein1971-ed	refs.bib	/^@BOOK{Stein1971-ed,$/;"	e
Sun, Weiwei and Tagliasacchi, Andrea and Deng, Boyang and Sabour, Sara and Yazdani, Soroosh and Hinton, Geoffrey E and Yi, Kwang Moo	refs.bib	/^  author={Sun, Weiwei and Tagliasacchi, Andrea and Deng, Boyang and Sabour, Sara and Yazdani, So/;"	a
Sun2020-mu	refs.bib	/^@article{Sun2020-mu,$/;"	e
Sutton, Charles and McCallum, Andrew	refs.bib	/^  author    = "Sutton, Charles and McCallum, Andrew",$/;"	a
Sutton2012-fe	refs.bib	/^@ARTICLE{Sutton2012-fe,$/;"	e
Szeliski, Richard	refs.bib	/^  author    = "Szeliski, Richard",$/;"	a
Szeliski2007-ul	refs.bib	/^@ARTICLE{Szeliski2007-ul,$/;"	e
T. M. Mitchell	example/example_paper.bib	/^  author = 	 "T. M. Mitchell",$/;"	a
Vural, Elif and Frossard, Pascal	refs.bib	/^  author    = "Vural, Elif and Frossard, Pascal",$/;"	a
Vural2014-xr	refs.bib	/^@ARTICLE{Vural2014-xr,$/;"	e
Weiler, Maurice and Cesa, Gabriele	refs.bib	/^  author    = "Weiler, Maurice and Cesa, Gabriele",$/;"	a
Weiler2019-bx	refs.bib	/^@INPROCEEDINGS{Weiler2019-bx,$/;"	e
Weiler2021-ps	refs.bib	/^@ARTICLE{Weiler2021-ps,$/;"	e
Wiatowski2018-qr	refs.bib	/^@ARTICLE{Wiatowski2018-qr,$/;"	e
Worrall, Daniel E. and Garbin, Stephan J. and Turmukhambetov, Daniyar and Brostow, Gabriel J.	refs.bib	/^author = {Worrall, Daniel E. and Garbin, Stephan J. and Turmukhambetov, Daniyar and Brostow, Gab/;"	a
Worrall_2017_CVPR	refs.bib	/^@InProceedings{Worrall_2017_CVPR,$/;"	e
Xiao2018-eq	refs.bib	/^@INPROCEEDINGS{Xiao2018-eq,$/;"	e
Yenson Lau and Qing Qu and Han-Wen Kuo and Pengcheng Zhou and Yuqian Zhang and John Wright	refs.bib	/^author={Yenson Lau and Qing Qu and Han-Wen Kuo and Pengcheng Zhou and Yuqian Zhang and John Wrig/;"	a
Zaitsev, Maxim and Maclaren, Julian and Herbst, Michael	refs.bib	/^  author   = "Zaitsev, Maxim and Maclaren, Julian and Herbst, Michael",$/;"	a
Zaitsev2015-ot	refs.bib	/^@ARTICLE{Zaitsev2015-ot,$/;"	e
alg:example	example/example_paper.tex	/^   \\label{alg:example}$/;"	l
alg:hier_detection	sections/hier_detect.tex	/^  \\label{alg:hier_detection}$/;"	l
anonymous	example/example_paper.bib	/^@misc{anonymous,$/;"	e
app:mc-spike-affine	main.tex	/^\\section{Proof of \\Cref{thm:multichannel-spike}} \\label{app:mc-spike-affine}$/;"	l
ass:xfinite	example/example_paper.tex	/^\\label{ass:xfinite}$/;"	l
author info	example/example_paper.tex	/^\\label{author info}$/;"	l
def:inj	example/example_paper.tex	/^\\label{def:inj}$/;"	l
e2018matrix	refs.bib	/^@inproceedings{e2018matrix,$/;"	e
eq:affine_subspace	sections/app_implementation.tex	/^    \\label{eq:affine_subspace}$/;"	l
eq:affine_subspace_centered	sections/app_implementation.tex	/^  \\label{eq:affine_subspace_centered}$/;"	l
eq:complementary_smoothing	sections/hier_detect.tex	/^  \\label{eq:complementary_smoothing}$/;"	l
eq:cov_differential	sections/app_implementation.tex	/^      \\labelthis \\label{eq:cov_differential}$/;"	l
eq:differential_term1	sections/app_implementation.tex	/^      \\label{eq:differential_term1}$/;"	l
eq:differential_term2	sections/app_implementation.tex	/^      \\label{eq:differential_term2}$/;"	l
eq:differential_term3	sections/app_implementation.tex	/^      \\label{eq:differential_term3}$/;"	l
eq:formulation_costsmooth	sections/approach.tex	/^  \\label{eq:formulation_costsmooth}$/;"	l
eq:formulation_reg	sections/approach.tex	/^  \\label{eq:formulation_reg}$/;"	l
eq:formulation_withbg	sections/approach.tex	/^  \\label{eq:formulation_withbg}$/;"	l
eq:general_formulation	sections/approach.tex	/^  \\label{eq:general_formulation}$/;"	l
eq:hier_strided_occmaps	sections/hier_detect.tex	/^  \\label{eq:hier_strided_occmaps}$/;"	l
eq:hier_strided_spiky	sections/hier_detect.tex	/^  \\label{eq:hier_strided_spiky}$/;"	l
eq:hier_strided_textured	sections/hier_detect.tex	/^  \\label{eq:hier_strided_textured}$/;"	l
eq:linked_rigid_body_1level	sections/hier_detect.tex	/^  \\label{eq:linked_rigid_body_1level}$/;"	l
eq:linked_rigid_body_1level_obs	sections/hier_detect.tex	/^  \\label{eq:linked_rigid_body_1level_obs}$/;"	l
eq:linked_rigid_body_dlevel_obs	sections/hier_detect.tex	/^  \\label{eq:linked_rigid_body_dlevel_obs}$/;"	l
eq:logdet_differential	sections/app_implementation.tex	/^      \\label{eq:logdet_differential}$/;"	l
eq:matrix_inv_differential	sections/app_implementation.tex	/^      \\label{eq:matrix_inv_differential}$/;"	l
eq:mcs_inverse_param	sections/mcs_theory.tex	/^ \\label{eq:mcs_inverse_param}$/;"	l
eq:multichannel_spike_map	sections/hier_detect.tex	/^  \\label{eq:multichannel_spike_map}$/;"	l
eq:opt-main-boundmain	sections/mcs_theory.tex	/^    \\mb A_\\star \\|_{F}^2 + \\| \\mb b_\\star \\|_{2}^2 \\Bigr), \\label{eq:opt-main-boundmain/;"	l
eq:projection_onto_aff	sections/app_implementation.tex	/^  \\label{eq:projection_onto_aff}$/;"	l
eq:prox_general	sections/approach.tex	/^  \\label{eq:prox_general}$/;"	l
eq:registration_unrolled	sections/approach.tex	/^  \\label{eq:registration_unrolled}$/;"	l
eq:sigma-bound	sections/mcs_theory.tex	/^    \\label{eq:sigma-bound}$/;"	l
eq:spike_reg_stepsizes	sections/mcs_theory.tex	/^    \\label{eq:spike_reg_stepsizes}$/;"	l
eqn:M-bound	sections/app_proofs.tex	/^&\\le& 1 - \\frac{1}{\\kappa} + 2 \\| \\nu \\dot{\\mb \\psi} - \\One\\|_{\\ell^\\infty}, \\label/;"	l
eqn:MCSM-spike-rel	sections/app_proofs.tex	/^\\begin{equation} \\label{eqn:MCSM-spike-rel}$/;"	l
eqn:MCSM-spike-rel	sections/mcs_theory.tex	/^\\begin{equation*}% \\label{eqn:MCSM-spike-rel}$/;"	l
eqn:X-MCSM	sections/app_proofs.tex	/^\\begin{equation} \\label{eqn:X-MCSM}$/;"	l
eqn:X-MCSM	sections/mcs_theory.tex	/^\\begin{equation*}% \\label{eqn:X-MCSM}$/;"	l
eqn:X0-MCSM	sections/app_proofs.tex	/^\\begin{equation} \\label{eqn:X0-MCSM}$/;"	l
eqn:X0-MCSM	sections/mcs_theory.tex	/^\\begin{equation*}% \\label{eqn:X0-MCSM}$/;"	l
eqn:delta-bound	sections/app_proofs.tex	/^   \\ell^2} }. \\label{eqn:delta-bound}$/;"	l
eqn:one-iter	sections/app_proofs.tex	/^    &\\doteq& \\mb M \\left[ \\begin{array}{c} \\mr{vec}(\\bar{\\mb \\Delta}_{\\mb A}) \\\\ \\ba/;"	l
eqn:opt-main-bound	sections/app_proofs.tex	/^    t_{\\mb A}^{-1} \\| \\mb A_k - \\mb A_\\star \\|_{F}^2 + \\| \\mb b_k - \\mb b_\\star \\|_2^/;"	l
eqn:psi-cond	sections/app_proofs.tex	/^\\begin{equation} \\label{eqn:psi-cond}$/;"	l
fig:architecture_registration	figs/registration/mockup/vis.tex	/^  \\label{fig:architecture_registration}$/;"	l
fig:basin	sections/experiments.tex	/^    \\label{fig:basin}$/;"	l
fig:centerpiece	sections/intro.tex	/^\\label{fig:centerpiece}$/;"	l
fig:convergence	sections/mcs_theory.tex	/^  \\label{fig:convergence}$/;"	l
fig:detection	sections/hier_detect.tex	/^  \\label{fig:detection}$/;"	l
fig:example	sections/other_applications.tex	/^    \\label{fig:example}$/;"	l
fig:motif	sections/approach.tex	/^  \\label{fig:motif}$/;"	l
fig:multispike	sections/app_implementation.tex	/^%    \\label{fig:multispike}$/;"	l
final author	example/example_paper.tex	/^\\label{final author}$/;"	l
icml-historical	example/example_paper.tex	/^\\label{icml-historical}$/;"	l
kearns89	example/example_paper.bib	/^@phdthesis{kearns89,$/;"	e
langley00	example/example_paper.bib	/^@inproceedings{langley00,$/;"	e
lem:usefullemma	example/example_paper.tex	/^\\label{lem:usefullemma}$/;"	l
mitchell80	example/example_paper.bib	/^@TechReport{mitchell80,$/;"	e
pmlr-v80-kondor18a	refs.bib	/^@InProceedings{pmlr-v80-kondor18a,$/;"	e
prop:complementary_smoothing_filter_grad	sections/app_implementation.tex	/^  \\label{prop:complementary_smoothing_filter_grad}$/;"	l
prop:inverse_parameterization	sections/app_implementation.tex	/^  \\label{prop:inverse_parameterization}$/;"	l
prop:reg_gradient	sections/app_implementation.tex	/^  \\label{prop:reg_gradient}$/;"	l
sample-table	example/example_paper.tex	/^\\label{sample-table}$/;"	l
sec:basin_details	sections/app_implementation.tex	/^%\\subsubsection{\\Cref{fig:basin} Experimental Details}\\label{sec:basin_details}$/;"	l
sec:basin_experiments	main.tex	/^\\Cref{eq:formulation_withbg}} \\label{sec:basin_experiments}$/;"	l
sec:examples	main.tex	/^%\\section{Examples} \\label{sec:examples}$/;"	l
sec:experiments	main.tex	/^%\\section{Learning Invariant Networks with Unrolled Optimization} \\label{sec:experiments}$/;"	l
sec:extra_experiment_details	sections/app_implementation.tex	/^\\subsection{Additional Experiments and Experimental Details} \\label{sec:extra_experiment_detai/;"	l
sec:formulations	sections/approach.tex	/^\\label{sec:formulations}$/;"	l
sec:framework	main.tex	/^\\label{sec:framework}$/;"	l
sec:grads	sections/app_implementation.tex	/^\\subsection{Gradient Calculations for Unrolled Network Architectures} \\label{sec:grads}$/;"	l
sec:hier_data_model	sections/hier_detect.tex	/^\\subsection{Data Model and Problem Formulation} \\label{sec:hier_data_model}$/;"	l
sec:hier_networks	sections/hier_detect.tex	/^\\subsection{Invariant Network Architecture} \\label{sec:hier_networks}$/;"	l
sec:hier_preprocessing	sections/app_implementation.tex	/^\\label{sec:hier_preprocessing}$/;"	l
sec:hier_results	sections/hier_detect.tex	/^\\subsection{Implementation and Evaluation} \\label{sec:hier_results}$/;"	l
sec:hierarchical	sections/app_implementation.tex	/^%\\label{sec:hierarchical}$/;"	l
sec:intro	main.tex	/^\\section{Introduction}\\label{sec:intro}$/;"	l
sec:mcs_experiments	sections/mcs_theory.tex	/^\\subsection{Experimental Verification} \\label{sec:mcs_experiments}$/;"	l
sec:motif	main.tex	/^\\section{Invariant Networks for Hierarchical Object Detection} \\label{sec:motif}$/;"	l
sec:parametric	sections/app_implementation.tex	/^\\label{sec:parametric} $/;"	l
sec:relwork	main.tex	/^\\section{Related Work}\\label{sec:relwork}$/;"	l
sec:spike_reg	sections/hier_detect.tex	/^\\label{sec:spike_reg}$/;"	l
sec:theory	main.tex	/^\\section{Guaranteed, Efficient Detection of Occurrence Maps} \\label{sec:theory}$/;"	l
sec:unrolling	sections/approach.tex	/^\\subsection{Invariant Networks from Unrolled Optimization} \\label{sec:unrolling}$/;"	l
submission	example/example_paper.tex	/^\\label{submission}$/;"	l
thm:bigtheorem	example/example_paper.tex	/^\\label{thm:bigtheorem}$/;"	l
thm:multichannel-spike	sections/mcs_theory.tex	/^\\begin{theorem}[Multichannel Spike Model, Affine Transforms, $L^2$] \\label{thm:multichannel-sp/;"	l
thm:spike_reg_app	sections/app_proofs.tex	/^\\begin{theorem}[Multichannel Spike Model, Affine Transforms, $L^2$] \\label{thm:spike_reg_app}$/;"	l

